Oracle-Efficient Online Learning and Auction Design

We consider the design of computationally efficient online learning algorithms in an adversarial setting in which the learner has access to an offline optimization oracle. We present an algorithm called Generalized Follow-the-Perturbed-Leader and provide conditions under which it is oracle-efficient while achieving vanishing regret. Our results make significant progress on an open problem raised by Hazan and Koren, who showed that oracle-efficient algorithms do not exist in general and asked whether one can identify properties under which oracle-efficient online learning may be possible. Our auction-design framework considers an auctioneer learning an optimal auction for a sequence of adversarially selected valuations with the goal of achieving revenue that is almost as good as the optimal auction in hindsight, among a class of auctions. We give oracle-efficient learning results for: (1) VCG auctions with bidder-specific reserves in single-parameter settings, (2) envy-free item pricing in multi-item auctions, and (3) s-level auctions of Morgenstern and Roughgarden for single-item settings. The last result leads to an approximation of the overall optimal Myerson auction when bidders' valuations are drawn according to a fast-mixing Markov process, extending prior work that only gave such guarantees for the i.i.d. setting. Finally, we derive various extensions, including: (1) oracle-efficient algorithms for the contextual learning setting in which the learner has access to side information (such as bidder demographics), (2) learning with approximate oracles such as those based on Maximal-in-Range algorithms, and (3) no-regret bidding in simultaneous auctions, resolving an open problem of Daskalakis and Syrgkanis.

==> prelim.tex <==
\section{Preliminaries}

We consider $n$ bidders participating in single-item auctions.\footnote{We extend our results to multi-item auctions in Section~\ref{sec: }. } Let $v_i\in[0,1]$ be the value of bidder $i$ for the item.
Auction $a$ takes as input a reported valuation profile, or \emph{bid} profile, $\vec b$ and returns a pair of functions $\vec x(\vec b)$ and $\vec p(\vec b)$, where for each $i\in [n]$, $x_i(\vec b) =1$ if bidder $i$ receives the item and $x_i(\vec b) =0$  otherwise, and $p_i(\vec b)$ is the price  that bidder $i$ has to pay. Then, the utility of bidder $i$ is $v_i x_i(\vec b) - p_i(\vec b)$.
In this work, we consider \emph{truthful auctions}, where it is best for each bidder $i$ to report his true value $v_i$ irrespective of  what other bidders report, i.e., $\vec v = \vec b$. In the remainder of this work, we refer to $\vec v$ as the \emph{valuation profile} or \emph{bid profile} interchangeably. For each auction $a$ and bid profile $\vec v$, we denote by $\rev(a, \vec v)$ the \emph{revenue} of the auction that is the sum of the prices paid by the bidders, i.e., $\rev (a, \vec v) = \sum_{i\in[n]} p_i(\vec v)$.  

We consider the problem of learning auctions with optimal revenue for an online sequence of valuation profiles.





{\color{red}
Given a distribution $P$ over the valuation profiles, ........

Online problem. .......

We consider computationally efficient methods for the online problem. 


We consider the problem of choosing an auction within a set of auction that maximizes the revenue for a given a incoming sequence of valuation profiles. 

We consider class of truthful auctions, $\emph{Individual reserves}$,
$t$-level auctions, and hypergraph pricing auctions. In each case, we
defer the definition of each class of auctions to the respective
sections.
}



==> universal.tex <==
\subsection{Universal Identification Sequences}
\label{sec:universal}

Our definitions of admissibility and implementability are related to a statistical measure of complexity from learning theory, called the \emph{Universal Identification Sequences}.


\begin{definition}[Universal Identification Sequences~\cite{goldman1993exact}]
Consider a domain $\Z$ and a class of functions $\mathcal{H}$ mapping $\Z$ to $\{0,1\}$.
A set of unlabeled instances $\Z' \subseteq \Z$ is said to \emph{distinguish} a function $h\in\setH$ if $h$ is the only function that is consistent with the labeling on $\Z'$ produced by $h$.
A set of unlabeled instances $\Z'$ is called a \emph{universal identification sequence} if it distinguishes every $h\in\setH$.
\end{definition}

\nhedit{We note that the definition of \emph{Universal Identification Sequences} coincides with that of \emph{Separators} defined in \Sec{separable}, when we view $\Z$ as a space of contexts and $\setH$ as a space of policies.}

Here, we consider a learning problem where $\setH$ is the set of learner's actions, $\Z$ is the set of adversary actions and the payoff is given by the evaluation operator $f_\eval(h,z)\coloneqq h(z)$.
Then any universal identification sequence $\Z'$ for $\setH$ can be used
to construct a translation matrix that is $1$-admissible and implementable with complexity $1$ for the learning problem $(\setH,\Z,f_\eval)$. 
Specifically, the matrix $\mGamma^{\setH}$ whose rows are indexed by $h\in\setH$ and columns indexed by $z\in\Z'$ such that $\mGamma^{\setH}_{h,z}=h(z)=f(h,z)$ is $1$-admissible from the definition
of the universal identification sequence and implementable with complexity $1$ using datasets $\{ (1, z)\}$.
Note that any learning problem $(\X,\Y,f)$ where $f$ only takes values in $\set{0,1}$ can be cast in this framework by setting $\Z=\Y$ and $\setH=\set{h_x}_{x\in\X}$ where $h_x(y)\coloneqq f(x,y)$.
Thus, the number of columns needed to create a translation matrix that is admissible and implementable for any binary payoff $f$ can be upper-bounded by the \emph{length of a universal identification sequence} \mdedit{for the corresponding
function class $\setH$}. Examples of function
classes \nhedit{where the length of the  universal identification sequences is polynomial in the number of variables include}
logarithmic-depth read-once majority formulas, logarithmic-depth read-once positive NAND formulas~\cite{goldman1993exact}, boolean conjunctios and dis junctions and discretized linear threshold functions~\cite{Syrgkanis2016}. The next corollary is a direct consequence of Theorems~\ref{thm:FTPL-U} and \ref{thm:imp}.

\mdcomment{Do we want to describe in more detail what these formula classes are? What does the polynomial-length mean in this context (polynomial in what)? Do we want to describe any separator examples from \cite{Syrgkanis2016}?}\nhcomment{Done}

\begin{corollary}\label{cor:universal}
Consider a domain $\Z$ and a class of binary functions $\setH$ with a universal identification sequence $\Z'$ of length $d$.
Let $D$ be the uniform distribution as described in Theorem~\ref{thm:FTPL-U}. Then,
the Oracle-Based Generalized FTPL algorithm with $D$ and datasets  that implement $\mGamma^{\setH}$
is oracle-efficient with per-round complexity
$\order(T+d)$ and has regret
\[ \E\left[ \max_{h \in \setH}  \sum_{t=1}^T h(z^{(t)}) - \sum_{t=1}^T h^{(t)}(z^{(t)}) \right] \leq  O(d \sqrt{T}).
\]
\end{corollary}

Our notions of admissibility and implementability in a sense generalize the notion of universal identification sequences by allowing arbitrary real-valued payoffs (rather than just binary) and allowing implementation
by weighted datasets (rather than just single examples). In our examples, we have leveraged both of these extensions to design oracle-efficient no-regret algorithms for various problem classes with real-valued losses.
